LoftUp: Learning a Coordinate-Based Feature Upsampler for Vision Foundation Models

Vision foundation models (VFMs) such as DINOv2 and CLIP have achieved impressive results on various downstream tasks, but their limited feature resolution hampers performance in applications requiring pixel-level understanding. Feature upsampling offers a promising direction to address this challenge. In this work, we identify two critical factors for enhancing feature upsampling: the upsampler architecture and the training objective. For the upsampler architecture, we introduce a coordinate-based cross-attention transformer that integrates the high-resolution images with coordinates and low-resolution VFM features to generate sharp, high-quality features. For the training objective, we propose constructing high-resolution pseudo-groundtruth features by leveraging class-agnostic masks and self-distillation. Our approach effectively captures fine-grained details and adapts flexibly to various input and feature resolutions. Through experiments, we demonstrate that our approach significantly outperforms existing feature upsampling techniques across various downstream tasks. Our code is released at https://github.com/andrehuang/loftup.

==> sec/figs/fig-loss-compute.tex <==
\begin{figure}[t]
     \centering
         \includegraphics[width=0.8\linewidth]{sec/figs/loss-compare.pdf}
    \caption{\textbf{Low-res loss cannot distinguish differente upsamplers well.} We compare the conceptual difference between our training objective and previous works. Specifically, FeatUp and LiFT both computed loss at a resolution much lower than the image resolution (1/16 to 1/8). By constructing pseudo-GT, we can compute losses at a high resolution. \textcolor{blue}{TODO: Add LiFT loss and LiFT upsampler. BTW: Is it redundant if we already have the other figure for loss comparison?} }
    \label{fig:loss-compute}
\end{figure}


==> sec/figs/fig-self-distlled-pseudo-gt.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{sec/figs/Self-distillation-loss.pdf}
    \caption{\textbf{Constructing self-distilled pseudo-GT.} We omit the VFM in the teacher branch for visualization purpose. }
    \label{fig:enter-label}
\end{figure}


==> sec/supplements_extra.tex <==
% \section{More Related Work}\label{appx:literature}

% Image super-resolution

% CARAFE


\section{More Implementation Details}\label{appx:application-detail}

\subsection{Training details of LoftUp}
Our LoftUp upsampler is a 2-block cross-attention transformer that incorporates high-res image inputs with coordinates using an additional convolutional layer and low-res VFM features as keys and values in the cross-attention layers. Each transformer block consists of 1 cross-attention layer and 1 feedforward layer as in ViT~\cite{dosovitskiy2020vit}.
To train LoftUp, we use a batch size of 8 and AdamW~\cite{loshchilov2017decoupled} optimizer with a learning rate of 1e-3  in Stage 1 and 1e-4 in Stage 2 for more stable improvement during self-distillation. 
In Stage 2, we take 2 random crops per image to construct $\text{crop}\bigl({I_{\text{HR}}}\bigr)$, and update the teacher upsampler's weights every 10 steps using the EMA of the student upsampler with a decay factor of 0.99.
In both stages, we use $\alpha=0.8$ for mask refinement when constructing pseudo-GT to balance sharp boundaries from masks and the fine-grained details from high-resolution features within each mask region. 
For all upsamplers, including our compared ones, we train for 1 epoch on a 1M-image subset of SA1B dataset~\cite{kirillov2023segment}.

\subsection{Task setups}

\boldparagraph{Semantic segmentation} 
Following~\cite{fu2024featup,hamilton2022unsupervised}, we perform semantic segmentation on coarse classes in COCO-Stuff~\cite{caesar2018coco} (27 classes) and Cityscapes~\cite{Cordts2016Cityscapes} (19 classes) and report mean Intersection-over-Union (mIoU) for each dataset. We train a linear decoder layer on upsampled features with a batch size of 8 and AdamW optimizer~\cite{loshchilov2017decoupled} with a learning rate of 1e-4 for 10 epochs.

\boldparagraph{Depth and normal estimation}
Following~\cite{el2024probing}, we evaluate depth and normal estimation using NAVI dataset~\cite{jampani2023navi} and train a DPT decoder head with 7 convolutional layers on top of the VFM features. We use a batch size of 8  and AdamW optimizer~\cite{loshchilov2017decoupled} with a learning rate of 5e-4 for 10 epochs.
Following prior works~\cite{eigen2014depth, el2024probing, fouhey2015single}, we report the root-mean-squared prediction error (RMSE) for both tasks and recall at $\delta_3$ for scale-invariant depth estimation and at 30$^{\circ}$ for normal estimation. Here $\delta_3$ is computed as the number of pixels whose ratio of depth prediction to groundtruth is less than $1.25^3$:
\begin{equation*}
\delta_3(d^{pr}, d^{gt}) = \frac{1}{N} \sum_{j \in N} \max \left(\frac{d_j^{pr}}{d_j^{gt}}, \frac{d_j^{gt}}{d_j^{pr}}\right) < 1.25^3,
\end{equation*}
where $d^{pr}$ is predicted depth and $d^{gt}$ is groundtruth depth.

\boldparagraph{Video object segmentation}
This task involves propagating an object segmentation mask across video frames, given the ground truth mask for the first frame. Following prior evaluation protocols~\cite{suri2024lift, jabri2020space}, we compute dense feature affinity maps between frames to track objects. Performance is assessed using three metrics: J Mean, F Mean, and J \& F Mean. Specifically, J Mean denotes the average Intersection-over-Union (IoU) between predicted segmentations and groundtruth masks, while F Mean represents the average F-score, measuring contour accuracy via precision and recall against groundtruth boundaries.We evaluate our method on the DAVIS validation set~\cite{Pont-Tuset_arXiv_2017_davis}, a popular benchmark for video object segmentation. The dataset comprises 30 videos of varying lengths, each containing between 1 and 4 objects.




\boldparagraph{Zero-shot Open-Vocabulary Segmentation} We incorporate upsampled VFM features into ProxyCLIP~\cite{lan2024proxyclip}, a state-of-the-art method for zero-shot open-vocabulary segmentation (OVSeg), and evaluate on three popular OVSeg benchmarks: COCO~\cite{lin2014microsoft}, Cityscapes~\cite{Cordts2016Cityscapes}, and ADE20K~\cite{zhou2017scene}. ProxyCLIP enhances CLIP features by leveraging spatial feature correspondence from VFMs as proxy attention, effectively inheriting the strong local consistency of VFMs while retaining CLIP's remarkable zero-shot transferability. Due to the high computational cost of proxy attention, we perform upsampling to 8$\times$ for all upsampling methods. We use CLIP ViT-B/16~\cite{radford2021learning} as the CLIP backbone, DINOv2-S/14~\cite{oquab2024dinov} as the proxy VFM, and set the input resolution to 336px, matching the resolution of the CLIP backbone. 


\boldparagraph{Interactive Segmentation} We adapt the SimpleClick~\cite{liu2023simpleclick} architecture to evaluate upsampled features. Specifically, we use a frozen VFM backbone and train a single-layer click encoder that directly adds to the image patch embedding, along with a three-layer convolutional decoder head on top of the upsampled features for interactive segmentation.
For training, we follow prior works~\cite{liu2023simpleclick, sofiiuk2022reviving} and use the SBD dataset~\cite{hariharan2011semantic} to train for 20 epochs with the normalized focal loss~\cite{sofiiuk2019adaptis, sofiiuk2022reviving}. We employ the Adam optimizer~\cite{kingma2014adam} with a learning rate of 5e-5  and a batch size of 8.
For evaluation, following common practice~\cite{liu2023simpleclick, sofiiuk2022reviving, kirillov2023segment}, we sample the first click point as the farthest point from the object boundary, and report the mean IoU of the predicted segmentation masks with the groundtruth, denoted as IoU@1 Click. We report results on three popular interactive segmentation benchmarks: GrabCut~\cite{rother2004grabcut}, Berkeley~\cite{martin2001berkeley}, and DAVIS~\cite{perazzi2016davis}.



\section{More Quantitative Results}\label{appx:more-exps}

\begin{table}[th]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cc|cc}
    \toprule
       Resolution & Upsampler & COCO & Cityscapes\\
       \midrule
     \multirow{4}{*}{224}   & NA  &  40.30& 30.79 \\
      & Bilinear    & 47.12  & 39.84 \\
       % & FeatUp  & 48.28 & 39.18 \\
       & FeatUp  & 52.08 & 33.50 \\
       % & CA layer & FeatUp & 55.89 & 41.77\\
     %   & CA transformer & FeatUp & 56.58 & 43.04 \\
     %   & CA layer & FeatUp+HR & 56.53& 41.73 \\
     %   & CA layer & FeatUp+HR+large data & 56.44 & 43.97\\
       % & CA transformer & FeatUp+HR & \textbf{50.94} &  \textbf{40.46}\\
       % & FITUp (stage-1) & 51.67 & 42.88 \\
       & LoftUp & \textbf{52.58} & \textbf{44.66} \\
         \midrule
  \multirow{4}{*}{448} & NA &  42.14 &37.36 \\
  & Bilinear  & 48.32& 45.58\\
  & FeatUp  &  52.55 & 40.00\\
   & LoftUp & \textbf{53.87}& \textbf{50.14} \\
 \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Comparison of feature upsampers when VFM is CLIP-B/16~\cite{radford2021learning}.}}
    \label{tab:clip}
\end{table}


\begin{table}[th]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cc|cc}
    \toprule
       Resolution & Upsampler & COCO & Cityscapes\\
       \midrule
  \multirow{4}{*}{224}      & NA  &  51.00 & 34.42\\
      & Bilinear    &  56.77 & 43.09\\
       & FeatUp  & 56.59  & 42.23\\
       & LoftUp & \textbf{58.36} & \textbf{46.98} \\
         \midrule
 \multirow{4}{*}{448}  &NA & 58.94 & 49.30\\
  &Bilinear & 62.29 & 57.42 \\
  & FeatUp &  62.18&  56.58\\
  & LoftUp & \textbf{63.55} & \textbf{60.83}\\ % Check Sine PE:  59.03 & 55.39
 \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Comparison of feature upsampers when VFM is RADIOv2.5-B~\cite{am-radio}.}}
    \label{tab:radio}
\end{table}

\begin{table*}[th]
    \centering
    \resizebox{0.9\linewidth}{!}{%
    \begin{tabular}{cc|ccccc}
    \toprule
    & & \multicolumn{2}{c}{Semantic Seg.} & \multicolumn{3}{c}{Keypoint Correspondence}  \\
       Model & Upsampler & COCO & Cityscapes& PCK@0.1& PCK@0.05 & PCK@0.01\\
       \midrule
     \multirow{5}{*}{CLIP}   & NA  &  40.30& 30.79 & 16.61 & 6.07 & 0.24\\
      & Bilinear    & 47.12  & 39.84 \\
       & FeatUp  & 52.08 & 33.50 \\
       & LoftUp (Stage1, $\alpha=0.8$) & \textbf{52.58} (52.28) & \textbf{44.66} (41.99) & 14.94 & 6.23 & 0.58 \\
       & LoftUp (Stage2, 100000, $\alpha=0.5$) & 52.47 & 42.60 & 11.33 & 4.69 & 0.44\\
        % & LoftUp (Stage2, $\alpha=0.5$) & 51.80 & 40.43 \\
         \midrule
    \multirow{3}{*}{SigLIP} & NA & 39.25 & 27.34& 14.08 & 5.21 & 0.22\\
      & LoftUp (Stage1, $\alpha=0.8$) & 50.93 & 39.80 & 11.57 & 4.58 & 0.30 \\
     & LoftUp (Stage2, $\alpha=0.5$) & 51.63 & 39.40 & 9.06 & 3.66 & 0.31\\
     \midrule
    \multirow{2}{*}{SigLIP2} & NA & 42.17& 29.34 & 18.37 & 6.85 & 0.30\\
     & LoftUp (Stage2, $\alpha=0.5$) & \textbf{57.00} & \textbf{45.94} & 14.40 & 6.61 & 0.67\\
    \midrule
    \multirow{4}{*}{DINOv2-S} & NA  & 51.21 & 36.54 & 39.29 & 18.36 & 0.92 \\
     & LiFT & 53.35& 35.80 & 37.78 &19.71& 1.61 \\
     & LoftUp (old model) &  & & 39.41  & 19.37&1.32\\ 
     & LoftUp (Stage2) & 61.11 & 53.10 & 29.80 & 14.69 & 1.63\\
    \midrule
     \multirow{2}{*}{DINOv2-B} & NA & 52.19 & 40.01 & 42.74 & 19.78 & 1.01\\
     & LoftUp (Stage2) & 58.95 & 52.65  & 28.51 & 12.77 & 0.96 \\
  % \multirow{4}{*}{448} & NA &  42.14 &37.36 \\
  % & Bilinear  & 48.32& 45.58\\
  % & FeatUp  &  52.55 & 40.00\\
  %  & LoftUp & \textbf{53.87}& \textbf{50.14} \\
 \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Comparison of feature upsampers.} \textcolor{blue}{It seems LoftUp's success on segmentation tasks is really at the cost of the degradation of point-level tasks --- we over-learn the ``semantics''.} And at some point, the segmentation performance is no longer improving, but point-level performance is still worsening... We clearly need a better balance.}
    \label{tab:new}
\end{table*}

\begin{table*}[th]
    \centering
    \resizebox{0.8\linewidth}{!}{%
    \begin{tabular}{cc|ccccccccc}
    \toprule
       Model & Upsampler & COCO& Cityscapes & ADE20K \\
       \hline
    MaskCLIP & NA & 17.45 & 24.95 & 14.16\\
    MaskCLIP & LoftUp & To train \\
       \midrule
    ProxyCLIP (DINOv2-S)  & NA & 25.70 & 34.38 & 19.50\\
    ProxyCLIP (DINOv2-S) & LoftUp & 27.82 & 38.82 & 21.29 \\
       \midrule
     \multirow{4}{*}{CLIP}   & NA  & 5.09 &5.04 & 2.85\\
       & FeatUp  &  \\
       & LoftUp (Stage1) & 6.50 & 5.70 & 3.49\\
       & LoftUp (Stage2, 100000, $\alpha=0.5$) &  2.82& 6.20 & 2.48  \\
        % & LoftUp (Stage2, $\alpha=0.5$) &  \\
    \midrule
     SigLIP & NA & 0.05 & 1.98& 0.12\\
    SigLIP & LoftUp \\
    \midrule
    SigLIP2 & NA \\
    SigLIP2 & LoftUp \\

 \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Open-Voc Experiments.} CLIP ViT-B backbone. No ProxyVFM, no MaskCLIP, CLIP final dense features only.}
    \label{tab:open-voc}
\end{table*}


\begin{table*}[th]
    \centering
    \resizebox{0.9\linewidth}{!}{%
    \begin{tabular}{cc|ccccccccc}
    \toprule
       Model & Upsampler & VOC & Context& COCO& Context59 & VOC20 & COCO Sutff & Cityscapes & ADE20K & avg\\
       \midrule
     \multirow{4}{*}{MaskCLIP}   & NA  & 32.87&22.87&16.33&25.53&61.79&17.45&24.95&14.16&26.99\\
       & FeatUp  &  \\
       & LoftUp (Stage1) &  27.32 & 9.84 & 7.45 & 10.40 & 38.08 & 3.58 & 6.83 & 3.00 & 13.31\\
       & LoftUp (Stage2, 100000, $\alpha=0.5$) & 4.83 & 2.65 & 0.34 & 2.85 & 5.64 & 0.32 & 1.27 & 0.44 & 2.29\\
        % & LoftUp (Stage2, $\alpha=0.5$) &  \\
             %  SigLIP & LoftUp (Stage1) & \\
    % SigLIP & LoftUp (Stage2) & \\
    % SigLIP2 & LoftUp (Stage2) & retrain\\


 \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Open-Voc Experiments.} CLIP ViT-B backbone. \textcolor{blue}{Note currently, the LoftUp was not trained for MaskCLIP, but on CLIP dense features.} \textcolor{red}{TODO: Train a new upsampler on MaskCLIP features.}}
    \label{tab:open-voc}
\end{table*}

\boldparagraph{Upsampling CLIP and RADIO} In~\cref{tab:clip} and~\cref{tab:radio}, we compare LoftUp with FeatUp and a bilinear upsampling baseline using CLIP~\cite{radford2021learning} and RADIO~\cite{am-radio} as VFM backbones. The upsamplers are trained following the same procedure as on the DINOv2 backbone and evaluated at resolutions 224 and 448. As with DINOv2, LoftUp consistently outperforms all baselines when using CLIP and RADIO as VFM backbone, demonstrating the general applicability of our approach across different VFMs.




\boldparagraph{Ablation on the architecture and training data size} In~\cref{tab:arch-ablation}, we conduct an ablation study on both the architecture components of LoftUp and the training data size. For convenience, the upsamplers are trained using only the Stage 1 training objective.
Specifically, in experiment (a), we demonstrate that employing a sinusoidal positional encoding for the low-resolution features—combined with a 3x3 convolutional layer to process the high-resolution coordinates and image inputs—yields improved performance. This result is in line with prior work showing that sinusoidal positional encodings excel in coordinate-based methods~\cite{yu2020pixelnerf, mildenhall2021nerf, Ye_2023_featurenerf} and that stronger image processing layers help better integrate high-resolution information.
In experiment (b), we observe that two blocks of the cross-attention transformer are sufficient for optimal feature upsampling, with performance saturating at greater depths. Finally, in experiment (c), we find that training with a larger dataset improves performance, although the benefits begin to diminish as the dataset size increases. Consequently, we select a 1M-subset of the SA1B dataset~\cite{kirillov2023segment} to achieve the best balance among data diversity, model performance, and training time.


\input{sec/tables/tab-arch-ablation}

% \input{ICCV2025-Author-Kit-Feb/sec/tables/tab-nyu}


\section{More Visualization}\label{appx:visualization}

We further provide more visualization examples of upsampled features of various methods in~\cref{fig:more-vis-feats}, more prediction examples in semantic segmentation, depth estimation, and video object segmentation in~\cref{fig:more-vis-preds} and~\cref{fig:vis-preds-video}, more examples of different pseduo-GT in~\cref{fig:more-pseudo-gt}, and more examples of the attended regions of a high-resolution pixel in~\cref{fig:attn-map-supp}.

\input{sec/figs/fig-more-feats-vis}

\input{sec/figs/fig-more-pred-vis}

\input{sec/figs/fig-davis}
\input{sec/figs/fig-more-pseudo-gt}


\input{sec/figs/fig-attn-map-supp}


==> sec/tables/tab-interactive-seg.tex <==
\begin{table}[]
  \centering
  \resizebox{0.8\linewidth}{!}{%
  \begin{tabular}{l|cccc}
  \toprule
    Method & GrabCut & Berkeley & DAVIS & SBD  \\
     \midrule
%  No & 17.45 & 24.95 & 14.16 \\
% %  CLIP B/16   & No + JBU FeatUp&  20.61& 29.52&17.42\\
% \midrule
 Low-res & 64.90 & 55.77 & 52.82 & \\
 Bilinear &65.04 & 55.83& 54.26& 44.58\\
 LiFT & 29.66 & 31.99& 41.14 & \\
 FeatUp &65.89& 56.67& 55.03& 43.78\\

LoftUp & \textbf{78.49} & \textbf{65.24} & \textbf{67.31} & \textbf{50.22}\\
       \bottomrule
  \end{tabular}
  }
  \vspace{0.1cm}
  \caption{\textbf{Interactive Segmentation} using SimpleClick with frozen DINOv2 backbone. We report IoU@1 Click. }
  \label{tab:interactive-seg}
\end{table}

==> sec/tables/tab-more-tasks.tex <==
\begin{table*}[ht]
  \centering
  % First table
  \begin{minipage}{0.32\textwidth}
    % \centering
    \resizebox{\linewidth}{!}{%
      \begin{tabular}{l|cccc}
  \toprule
    Method & J Mean & F Mean & J \& F Mean  \\
     \midrule
%  No & 17.45 & 24.95 & 14.16 \\
% %  CLIP B/16   & No + JBU FeatUp&  20.61& 29.52&17.42\\
% \midrule
 Low-res & 42.05 & 31.27 & 36.66\\
Bilinear &42.62 & 33.90 & 38.26 \\
LiFT & 47.68 & 36.78 & 42.23 \\
FeatUp &45.70 & 42.90 & 44.30\\
%  DINOv2 + Ours (old) & 27.03  & 37.67 & 20.54 \\
% FITUp & \textbf{54.51} & \textbf{55.68} & \textbf{55.10}\\
\textbf{LoftUp} & \textbf{58.72} & \textbf{61.79} & \textbf{60.25}\\
% DINOv2 + Ours &\textbf{27.39} & \textbf{38.24} & \textbf{20.74} \\
       \bottomrule
  \end{tabular}
  }
    \caption{\textbf{Video Object Segmentation on DAVIS.}}
  \end{minipage}
  \hfill
  % Second table
  \begin{minipage}{0.3\textwidth}
    % \centering
    \resizebox{\linewidth}{!}{%
     \begin{tabular}{l|cccc}
  \toprule
    Method & COCO Stuff & CS & ADE  \\
     \midrule
%  No & 17.45 & 24.95 & 14.16 \\
% %  CLIP B/16   & No + JBU FeatUp&  20.61& 29.52&17.42\\
% \midrule
 Low-res & 25.70 & 34.48 & 19.50\\
 Bilinear & 25.78 & 34.56 & 19.53 \\
 LiFT & 25.96& 35.39& 19.50 \\
 FeatUp &26.61 & 35.01 &  19.99\\
%  DINOv2 + Ours (old) & 27.03  & 37.67 & 20.54 \\
% FITUp &\textbf{27.54} & \textbf{38.04} & \textbf{20.78} \\
\textbf{LoftUp} & \textbf{27.82} & \textbf{38.82} & \textbf{21.29} \\
% DINOv2 + Ours &\textbf{27.39} & \textbf{38.24} & \textbf{20.74} \\
       \bottomrule
  \end{tabular}
  }
    \caption{\textbf{Zero-Shot Open-Vocabulary Segmentation using ProxyCLIP.}}
  \end{minipage}
  \hfill
  % Third table
  \begin{minipage}{0.35\textwidth}
    % \centering
    \resizebox{\linewidth}{!}{%
      \begin{tabular}{l|cccc}
  \toprule
    Method & GrabCut & Berkeley & DAVIS & SBD  \\
     \midrule
%  No & 17.45 & 24.95 & 14.16 \\
% %  CLIP B/16   & No + JBU FeatUp&  20.61& 29.52&17.42\\
% \midrule
 Low-res & 64.90 & 55.77 & 52.82 & \\
 Bilinear &65.04 & 55.83& 54.26& 44.58\\
 LiFT & 29.66 & 31.99& 41.14 & \\
 FeatUp &65.89& 56.67& 55.03& 43.78\\

\textbf{LoftUp} & \textbf{78.49} & \textbf{65.24} & \textbf{67.31} & \textbf{50.22}\\
       \bottomrule
  \end{tabular}
  }
    \caption{\textbf{Interactive Segmentation using SimpleClick.}}
  \end{minipage}
  
  % \caption{Three tables arranged side by side}
  \label{tab:more-tasks}
\end{table*}

==> sec/tables/tab-open-voc-seg.tex <==
\begin{table}[]
  \centering
  \resizebox{0.6\linewidth}{!}{%
  \begin{tabular}{l|cccc}
  \toprule
    Method & COCO Stuff & CS & ADE  \\
     \midrule
%  No & 17.45 & 24.95 & 14.16 \\
% %  CLIP B/16   & No + JBU FeatUp&  20.61& 29.52&17.42\\
% \midrule
 Low-res & 25.70 & 34.48 & 19.50\\
 Bilinear & 25.78 & 34.56 & 19.53 \\
 LiFT & 25.96& 35.39& 19.50 \\
 FeatUp &26.61 & 35.01 &  19.99\\
%  DINOv2 + Ours (old) & 27.03  & 37.67 & 20.54 \\
% FITUp &\textbf{27.54} & \textbf{38.04} & \textbf{20.78} \\
LoftUp & \textbf{27.82} & \textbf{38.82} & \textbf{21.29} \\
% DINOv2 + Ours &\textbf{27.39} & \textbf{38.24} & \textbf{20.74} \\
       \bottomrule
  \end{tabular}
  }
  \vspace{0.1cm}
  \caption{\textbf{Zero-Shot Open-Vocabulary Segmentation using ProxyCLIP.} ProxyCLIP uses the sliding window approach during inference. Resolution is 336. The default backbone is CLIP B/16. The default Proxy VFM is DINOv2 S/14 (``token'' features). The default upsampling multiple is 8x.}
  \label{tab:open-voc-seg}
\end{table}

==> sec/tables/tab-video-seg.tex <==

\begin{table}[]
  \centering
  \resizebox{0.6\linewidth}{!}{%
  \begin{tabular}{l|cccc}
  \toprule
    Method & J Mean & F Mean & J \& F Mean  \\
     \midrule
%  No & 17.45 & 24.95 & 14.16 \\
% %  CLIP B/16   & No + JBU FeatUp&  20.61& 29.52&17.42\\
% \midrule
 Low-res & 42.05 & 31.27 & 36.66\\
Bilinear &42.62 & 33.90 & 38.26 \\
LiFT & 47.68 & 36.78 & 42.23 \\
FeatUp &45.70 & 42.90 & 44.30\\
%  DINOv2 + Ours (old) & 27.03  & 37.67 & 20.54 \\
% FITUp & \textbf{54.51} & \textbf{55.68} & \textbf{55.10}\\
LoftUp & \textbf{58.72} & \textbf{61.79} & \textbf{60.25}\\
% DINOv2 + Ours &\textbf{27.39} & \textbf{38.24} & \textbf{20.74} \\
       \bottomrule
  \end{tabular}
  }
  \vspace{0.1cm}
  \caption{\textbf{DAVIS Video Object Segmentation.} }
  \label{tab:video-seg}
\end{table}
